Tackling the Objective Inconsistency Problem in Heterogeneous Federated Optimization

In federated optimization, heterogeneity in the clients' local datasets and computation speeds results in large variations in the number of local updates performed by each client in each communication round. Naive weighted aggregation of such models causes objective inconsistency, that is, the global model converges to a stationary point of a mismatched objective function which can be arbitrarily different from the true objective. This paper provides a general framework to analyze the convergence of federated heterogeneous optimization algorithms. It subsumes previously proposed methods such as FedAvg and FedProx and provides the first principled understanding of the solution bias and the convergence slowdown due to objective inconsistency. Using insights from this analysis, we propose FedNova, a normalized averaging method that eliminates objective inconsistency while preserving fast error convergence.

==> 4_analysis.tex <==
\section{New Theoretical Framework For Heterogeneous Federated Optimization}\label{sec:analysis}
% In previous federated optimization literature, it is common practice to use the virtual sequence technique \cite{stich2018local,yu2018parallel,wang2018cooperative,yu2019linear,Wang2020SlowMo,Li2020On,haddadpour2019convergence,haddadpour2019trading,haddadpour2019local,khaled2020tighter}. The update rule of \fedavg is formulated as $\overline{\bm{x}}^{(k+1)} = \overline{\bm{x}}^{(k)} -\lr\sum_{i=1}^\nworkers p_i\sg_i(\x_i^{(k)})$, where $\overline{\bm{x}}$ denotes the average of all local models and $k$ is the iteration index. However, this approach cannot be trivially extended to the case when clients have heterogeneous local progress, because the iteration indices of clients are asynchronous. 

While \Cref{lem:quadratic} provides a simple intuition in quadratic model, in this section we are going to present a general theoretical framework to analyze and understand the objective inconsistency problem. While the main results are stated for non-convex and full client participation setting. It is fairly easy to extend the theorems to (strongly) convex or client sampling cases. %An example of such extension is provided in \Cref{sec:extension}.

\GJ{There is quite some redundancy in the equations (5)-(8) and the related discussion, which we can try to shorten}

\subsection{New Formulation of Federated Optimization Algorithms}
\textbf{Generalized Federated Optimization.} Recall that the update rule of federated optimization algorithms can be written as $\x^{(t+1,0)} = \x^{(t,0)} + \sum_{i=1}^\nworkers p_i \Delta_i^{(t)}$, where $\Delta_i^{(t)}:=\x^{(t,\cp_i)} - \x^{(t,0)}$ denote the local parameter changes of client $i$ at round $t$ and $p_i = n_i/n$, the fraction of data at client $i$. In this paper, we will focus on a class of client optimizers, in which the local change is a linear combination of stochastic gradients:
\begin{align}
    \Delta_i^{(t)}
    = -\lr \sum_{k=0}^{\cp_i-1}a_{i,k}\sg_i(\x_i^{(t,k)}) := -\lr \matG_i^{(t)}\gradweight_i, \label{eqn:delta}
\end{align}
where  $\matG_i^{(t)} = [\sg_i(\x_i^{(t,0)}), \sg_i(\x_i^{(t,1)}),\dots, \sg_i(\x_i^{(t,\cp_i)})] \in \mathbb{R}^{d \times \cp_i}$ stacks all stochastic gradients in the $t$-th round, $\lr$ is the initial local learning rate per round, and $\gradweight_i\in \mathbb{R}^{\cp_i}$ defines how stochastic gradients are locally accumulated. Note that each element in $\gradweight_i$ should be non-negative. When the local solver is SGD as in \fedavg, then $\gradweight_i=[1,1,\dots,1]\in\mathbb{R}^{\cp_i}$. By setting different $\gradweight_i$ vectors, \Cref{eqn:delta} works for most popular client optimizers, such as SGD with proximal term, SGD with local momentum, SGD with variable learning rate, etc. In Appendix, we provide detailed derivations on these examples.

In intuition, when a client performs more local updates than others, the relative scale of its local change $\Delta_i$ also increases. When the server aggregates the local changes from all clients, it will implicitly assign more weights to the direction that has a larger scale. As a result, the server model would be gradually biased towards the fast client. In order to formulate this intuition, we propose the following general update rule for federated optimization algorithms:
\begin{align}
    \x^{(t+1,0)} - \x^{(t,0)} = - \cpeff \sum_{i=1}^\nworkers w_i \cdot \lr \nsg_i^{(t)}, \quad \text{where} \ \nsg_i^{(t)} = \frac{\matG_i^{(t)}\gradweight_i}{\|\gradweight_i\|_1}, \ \sum_{i=1}^\nworkers w_i = 1. \label{eqn:new_update}
\end{align}
In the above formulation, we define $\nsg_i$ as the \emph{normalized gradient}, because it is a weighted average of the gradients. Besides, $\|\gradweight_i\|_1$ is just a summation of all elements of $\gradweight_i$, which is a non-negative vector. The aggregated normalized gradient is re-scaled by a constant $\cpeff$, named \emph{effective local steps}. Intuitively, it is a kind of statistic of clients local progress and indicates how many gradient steps the server model moves along with the aggregated direction. Later in Section 5, we will prove that any federated optimization algorithms following the updates \Cref{eqn:new_update} will converge to the stationary points of $\surloss(\x)=\sum_{i=1}^\nworkers w_i \obj_i(\x)$.
\begin{rem}
For the clarity of presentation, in \Cref{eqn:delta} and the following derivations, we let $\gradweight_i$ to be fixed at all rounds. Nonetheless, this formulation also works for the case when $\cp_i$ and $\gradweight_i$ are time-varying.
\end{rem}

\textbf{Previous Algorithms as Special Cases.} The above formulation is general enough to subsume most previous algorithms. One can validate this by rearranging \Cref{eqn:delta}. It follows that:
\begin{align}
    \x^{(t+1,0)} - \x^{(t,0)}
    =& \sum_{i=1}^\nworkers p_i \Delta_i^{(t)} = -\sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1  \cdot \frac{\lr \matG_i^{(t)}\gradweight_i}{\|\gradweight_i\|_1}\\
    =& - \underbrace{\parenth{\sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1}}_{\cpeff:\ \text{effective local steps}}\sum_{i=1}^\nworkers \lr \underbrace{\parenth{\frac{p_i\|\gradweight_i\|_1}{\sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1}}}_{w_i:\ \text{weight}}\underbrace{\parenth{\frac{\matG_i^{(t)}\gradweight_i}{\|\gradweight_i\|_1}}}_{\nsg_i:\ \text{normalized gradient}} \label{eqn:new_form1}
\end{align}
Comparing \Cref{eqn:new_update,eqn:new_form1}, observe that if one averages the local changes as previous algorithms, then not only the weight of normalized gradient but also the effective local steps are implicitly influenced by the local solver (\ie, the choice of $\gradweight_i$). Here, we provide few examples to illustrate the problem.
\begin{itemize}[wide, labelwidth=!, labelindent=0pt]
\item In \fedavg, the local solver is SGD such that $\gradweight_i = [1,1,\dots,1]\in\mathbb{R}^{\cp_i}$ and $\|\gradweight_i\|=\cp_i$. As a consequence, the normalized gradient $\nsg_i$ is a simple average over $\cp_i$ iterations, $\cpeff=\sum_{i=1}^\nworkers p_i \cp_i$, and $w_i = p_i \cp_i/\sum_{i=1}^\nworkers p_i \cp_i$. That is, the normalized gradients with more local steps will be assigned with higher weights.
\item In \fedprox, local SGD steps are corrected by a penalty term. It can be shown that $\gradweight_i = [(1-\alpha)^{\cp_i-1},(1-\alpha)^{\cp_i-2},\dots,(1-\alpha),1]\in\mathbb{R}^{\cp_i}$, where $\alpha=\lr\mu$ and $\mu\geq 0$ is the penalty parameter. In this case, we have 
\begin{align}
    \cpeff = \frac{1}{\alpha}\sum_{i=1}^\nworkers p_i [1-(1-\alpha)^{\cp_i}], \quad w_i = \frac{p_i [1-(1-\alpha)^{\cp_i}]}{\sum_{i=1}^\nworkers p_i [1-(1-\alpha)^{\cp_i}]}. \label{eqn:fedprox_w}
\end{align}
Compared to \fedavg, although the weight of \fedprox is more similar to $p_i$, its effective local steps becomes smaller. At an extreme case $\alpha=1$, then $\cpeff=1$, which is much smaller than the case of \fedavg and will greatly slow down the convergence. We will formally discuss this trade-off via our convergence analysis in the next subsection.
\item More generally, \Cref{eqn:new_form1} suggests that $w_i \neq p_i$ as long as clients have different $\|\gradweight_i\|_1$, which may be caused by imbalanced local updates (\ie, $\gradweight_i$'s have different dimensions), or various local learning rate / momentum sequence (\ie, $\gradweight_i$'s have different scales). For instance, when clients' local learning rates are exponentially decayed but in different speeds, we have $\gradweight_i=[\gamma_i,\gamma_i^2, \dots,\gamma_i^{\cp_i}]$ where $\gamma_i \geq 0$.
\end{itemize}

% For example, 



% \begin{align}
%     \x^{(t+1,0)} - \x^{(t,0)} = - \cpeff \sum_{i=1}^\nworkers w_i \cdot \lr \nsg_i^{(t)}
% \end{align}


% \textbf{Allow Heterogeneous Local Progress by Setting $\gradweight_i$.} The above formulation is general enough to subsume most popular configurations of local optimizers. The use of $\gradweight_i$ vector gives clients the flexibility to have heterogeneous local progress. Beyond different local steps, each client can also choose arbitrary local learning rate sequence, add local proximal terms as \fedprox, or even maintain separate local momentum buffers. All of these will result in heterogeneous local progress at clients but can be easily taken into account in the novel formulation by setting different $\gradweight_i$ vectors. For instance, when clients run local SGD with fixed step sizes as \fedavg, we have $\gradweight_i = [1,1,\dots,1]\in\mathbb{R}^{\cp_i}$; when the local learning rate is diminishing, we have $\gradweight_i=[\gamma_i,\gamma_i^2, \dots,\gamma_i^{\cp_i}]$ for some $0<\gamma_i<1$; in \fedprox, stochastic gradient are corrected by a penalty term. One can show that $\gradweight_i = [(1-\alpha)^{\cp_i-1},(1-\alpha)^{\cp_i-2},\dots,(1-\alpha),1]\in\mathbb{R}^{\cp_i}$, where $\alpha=\lr\mu$ and $\mu$ is the penalty parameter. 

% To see this, we can expand the local changes as follows:
% \begin{align}
    % \Delta_i^{(t)} 
    % =  \x^{(t,\cp_i)} - \x^{(t,0)}
    % =& \x^{(t,\cp_i-1)} -\lr\brackets{\sg_i(\x^{(t,\cp_i-1)}) +\mu(\x_i^{(t,\cp_i-1)}-\x^{(t,0)})} - \x^{(t,0)} \\
    % =& -\lr\sg_i(\x^{(t,\cp_i-1)}) + (1-\lr\mu)(\x_i^{(t,\cp_i-1)}-\x^{(t,0)}).
% \end{align}
% Repeating the above procedure, it follows that $\Delta_i^{(t)} = -\lr \sum_{k=0}^{\cp_i-1} (1-\lr\mu)^{\cp_i-1-k}\sg_i(\x_i^{(t,k)}) = -\lr\matG_i\gradweight_i$. When clients optimize local objectives using momentum, then $\gradweight_i =[1-\rho^{\cp_i},1-\rho^{\cp_i-1},\dots,1-\rho]/(1-\rho)$, where $\rho$ is the momentum factor. In Appendix we provide detailed derivations. %Except \fedavg with fixed local learning rate, none of these instances are analyzed in previous literature.

% \begin{table}[!htbp]
% \caption{}
% \centering
% \begin{tabular}{*2c}    \toprule
% Configurations of Local SGD & Gradient weights $\gradweight_i$ in \Cref{eqn:delta}\\\midrule
% Fixed step size (\fedavg \cite{mcmahan2016communication}) & $[1,1,\dots,1]$ \\
% Decaying step size & $[1,\gamma,\dots,\gamma^{\cp_i-1}]$ \\
% Add proximal term (\fedprox \cite{sahu2018convergence}) & $[(1-\lr\mu)^{\cp_i-1},\dots,(1-\lr\mu),1]$ \\
% \bottomrule
% \end{tabular}
% \label{tab:comp}
% \end{table}

% \textbf{Equivalent Update Rule for the Server Model.} Rearranging \Cref{eqn:delta}, the sever model is equivalently updated by the following quantity:
% \begin{align}
%     \sum_{i=1}^\nworkers p_i \Delta_i^{(t)}
%     =& - \underbrace{\parenth{\sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1}}_{\cpeff:\ \text{effective local steps}}\sum_{i=1}^\nworkers \lr \underbrace{\parenth{\frac{p_i\|\gradweight_i\|_1}{\sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1}}}_{w_i:\ \text{weight}}\underbrace{\parenth{\frac{\matG_i^{(t)}\gradweight_i}{\|\gradweight_i\|_1}}}_{\nsg_i:\ \text{normalized gradient}} \label{eqn:new_form1}
% \end{align}
% where $\|\gradweight_i\|_1$ is the $\ell_1$ norm of vector $\gradweight_i$. Since all elements in $\gradweight_i$ are non-negative, the $\ell_1$ norm equals to the summation of all elements. In this new formulation \Cref{eqn:new_form1}, it is worth highlighting three key terms. Firstly, we define $\nsg_i=\matG_i\gradweight_i/\|\gradweight_i\|_1$ as the \emph{normalized stochastic gradient}. In \fedavg, $\nsg_i^{(t)} = \frac{1}{\cp_i}\sum_{k=0}^{\cp_i-1}\sg_i(\x_i^{(t,k)})$ is just the simple average of all stochastic gradients in the current round. %In other cases, $\nsg_i$ is a weighted average of current round's gradients.

% Secondly, observe that, in previous algorithms even though the local changes $\Delta_i$'s are averaged in proportion to the local data size $p_i$, the normalized gradients $\nsg_i$'s are actually averaged in a biased way. The weight of $\nsg_i$ is $w_i\propto p_i \|\gradweight_i\|_1$ instead of $p_i$. In next subsection, we will prove that the biased averaging is the main cause of objective inconsistency. That is, previous algorithms actually converge to the stationary points of a surrogate objective function $\surloss(\x) = \sum_{i=1}^\nworkers w_i \obj_i(\x)$, though they aim at optimizing the original one $\obj(\x)=\sum_{i=1}^\nworkers p_i\obj_i(\x)$.

% Lastly, in \Cref{eqn:new_form1}, the aggregated normalized gradient is re-scaled by a constant $\cpeff = \sum_{i=1}^\nworkers p_i \|\gradweight_i\|_1$, named \emph{effective local steps}. Intuitively, it indicates how much the server model moves along with the aggregated direction. In \fedavg, $\cpeff=\sum_{i=1}^\nworkers p_i \cp_i$ is a weighted average of all local steps. In \fedprox, the value of $\cpeff$ is controlled by the penalty parameter $\mu$. Later we will prove that although a larger $\mu$ can mitigate the objective inconsistency, it makes $\cpeff$ become smaller and hence, results in slower convergence.

% As shown in \Cref{eqn:new_form1}, in previous algorithms, not only the weights $w_i$ but also the effective local steps $\cpeff$ are unnecessarily influenced by the choice of gradient accumulation method (\ie, the choice of vector $\gradweight_i$). However, \Cref{eqn:new_form1} naturally allows the use of other parameter choices. We can rewrite the server update rule as follows:
% \begin{align}
%     \x^{(t+1,0)} - \x^{(t,0)}
%     = -\cpeff \sum_{i=1}^\nworkers w_i \cdot \lr\nsg_i^{(t)}. \label{eqn:new_form2}
% \end{align}
% In the following, we will present a new convergence theory for the general updates \Cref{eqn:new_form2} and discuss the disadvantages of previous federated optimization algorithms as special cases.

% \begin{rem}
% In previous federated optimization literature, it is common practice to use the virtual sequence technique \cite{stich2018local,yu2018parallel,wang2018cooperative,yu2019linear,Wang2020SlowMo,Li2020On,haddadpour2019convergence,haddadpour2019trading,haddadpour2019local,khaled2020tighter}. The update rule of \fedavg is formulated as $\overline{\bm{x}}^{(k+1)} = \overline{\bm{x}}^{(k)} -\lr\sum_{i=1}^\nworkers p_i\sg_i(\x_i^{(k)})$, where $\overline{\bm{x}}$ denotes the average of all local models and $k$ is the iteration index. However, this approach cannot be trivially extended to the case when clients have heterogeneous local progress, as the iteration indices of clients are asynchronous. Some clients can perform much more gradient evaluations than others.
% \end{rem}



% In order to analysis the convergence of federated optimization algorithms, most of previous works focus on the convergence of a \emph{virtual sequence} $\overline{\x}^{(t,k)} = \sum_{i=1}^\nworkers p_i \x_i^{(t,k)}$, see \cite{stich2018local,yu2018parallel,wang2018cooperative,Li2020On,haddadpour2019convergence}. However, this method is infeasible when considering different local steps, since the iteration indices $(t,k)$ of clients are no longer synchronous to each other. Even when considering the same local steps but different local step sizes, one has to make non-trivial changes to the proofs.


==> 7_broader_impacts.tex <==
\section{Broader Impact}

The future of machine learning lies in moving both data collection as well as model training to the edge. This nascent research field called federated learning considers a large number of resource-constrained devices such as cellphones or IoT sensors that collect training data from their environment. Due to limited communication capabilities as well as privacy concerns, these data cannot be directly sent over to the cloud. Instead, the nodes locally perform a few iterations of training and only send the resulting model to the cloud. In this paper, we develop a federated training algorithm that is system-aware (robust and adaptable to communication and computation variabilities by allowing heterogeneous local progress) and data-aware (can handle skews in the size and distribution of local training data by correcting model aggregation scheme). This research has the potential to democratize machine learning by transcending the current centralized machine learning framework. It will enable lightweight mobile devices to cooperatively train a common machine learning model while maintaining control of their training data. 
